Unlocking the Capabilities of Masked Generative Models for Image Synthesis via Self-Guidance

Masked generative models (MGMs) have shown impressive generative ability while providing an order of magnitude efficient sampling steps compared to continuous diffusion models. However, MGMs still underperform in image synthesis compared to recent well-developed continuous diffusion models with similar size in terms of quality and diversity of generated samples. A key factor in the performance of continuous diffusion models stems from the guidance methods, which enhance the sample quality at the expense of diversity. In this paper, we extend these guidance methods to generalized guidance formulation for MGMs and propose a self-guidance sampling method, which leads to better generation quality. The proposed approach leverages an auxiliary task for semantic smoothing in vector-quantized token space, analogous to the Gaussian blur in continuous pixel space. Equipped with the parameter-efficient fine-tuning method and high-temperature sampling, MGMs with the proposed self-guidance achieve a superior quality-diversity trade-off, outperforming existing sampling methods in MGMs with more efficient training and sampling costs. Extensive experiments with the various sampling hyperparameters confirm the effectiveness of the proposed self-guidance.

==> sections/math.tex <==

Let $\Bar{\vx}_t$ be a perturbed sample that lacks some salient information $h_t$ from $\vx_t$. $h_t$ can be internal information within $\vx_t$ or an external condition, or both.
Given the salient information $h_t$, we aim to sample $\vx_t$ to maximize $p(\Bar{\vx}_t|h_t)$. However, for the correlation between the information and sample, $p(h_t|\Bar{\vx}_t)$ also needs to be as large as possible. 
For instance, if $h_t$ is defined as a class condition, $p(h_t|\vx_t)$ means the classification accuracy.
\begin{equation}
    % \argmax_{\vx_t} [\log p_\theta(\vx_t|h_t) + s (\log p_\theta(h_t|\vx_t))].
    \log p(\Bar{\vx}_t|h_t) + s \log p(h_t|\Bar{\vx}_t).
\end{equation}
Using the Bayes' theorem, the equation can be represented as
\begin{equation}
    % \argmax_{\vx_t} [\log p_\theta(\vx_t) + (1+s)(\log p_\theta(\vx_t|h_t) - \log p_\theta(\vx_t))].
    \log p(\Bar{\vx}_t) + (1+s)(\log p(\Bar{\vx}_t|h_t) - \log p(\Bar{\vx}_t)).
\end{equation}
If $h_t=c$ (class condition) and $\Bar{\vx}_t=\vx_t$, the equation collapses to classifier-free guidance (CFG), which guides the sampling toward the given class distribution.

One can assume $\Bar{\vx}_t \fallingdotseq \vx_{t+1}$ since the forward diffusion process degrades the input. 
Then the $h_t = \vx_{t} - \vx_{t+1}$ and joint probability $p(\Bar{\vx}_t|h_t)=p({\vx}_{t+1}|\vx_{t} - \vx_{t+1})$ can be simply converted to $p(\vx_t)$.
Then the equation is 
\begin{equation}
    \log p(\Tilde{\vx}_{t}) = \log p(\vx_{t+1}) + (1+s)(\log p(\vx_t) - \log p({\vx}_{t+1})).
\end{equation}
% \begin{equation} 

\begin{equation}
\begin{split}
    \log p(\Tilde{\vx}_{t+1}) &= \log p(\vx_{t+2}) + (1+s)(\log p(\vx_{t+1}) - \log p({\vx}_{t+2})) \\ 
    \log p(\Tilde{\vx}_{t}) &= \log p(\Tilde{\vx}_{t+1}) + (1+s)(\log p(\vx_t) - \log p(\Tilde{\vx}_{t+1}).
\end{split}
\end{equation}
Conceptually, this equation guides the sampling process toward the $h_t$, which means the contents generated by the reverse diffusion process. 
This term can enhance the consistency of the sampling.
Consistent sampling is known to help accurately estimate the score function and narrow the gap between the train and test (train-test discrepancy).
In Gaussian diffusion models, this equation is equivalent to the multi-step high-order sampling (DPM-Solver++(2M)) if we assume the guidance scale is timestep dependent i.e. $s=(2r_t)^{-1}$.

In the inference stage, discrete diffusion models estimate the marginal distribution $p(\vx_t)$ using the learned conditional sampler given samples from the previous step $p_\theta (\vx_t|\hat{\vx}_{t+1})$. 
Thus the logits with guidance are calculated as
\begin{equation}
    \log p(\Tilde{\vx}_{t}|\hat{\vx}_{t+1},\hat{\vx}_{t+2}) = \log p_\theta(\vx_{t+1}|\hat{\vx}_{t+2}) + (1+s)(\log p_\theta(\vx_{t}|\hat{\vx}_{t+1}) - \log p_\theta({\vx}_{t+1}|\hat{\vx}_{t+2}).
\end{equation}

In practice, to resemble the forward process $q(\vx_t)$, MGMs widely adopt two-step approach to estimate the $p(\vx_t)$.
However, we found that due to the stochastic sampling process of MGMs, $\hat{\vx}_t$ does not follow the distribution $p(\vx_t|\hat{\vx}_{t+1})$. The stochasticity are known to solve the multi-modality problem and setting appropriate temperature enhances the quality of samples and diversity simultaneously.
Thus, the prediction $\log p_\theta(\vx_{t}|\hat{\vx}_{t+1})$ and $\log p_\theta({\vx}_{t+1}|\hat{\vx}_{t+2})$ can have different predictions, especially when the sampling temperature is high, which increase the risk of sampling drift.

However, in a discrete diffusion model, using sampling temperature for diversity and solving multi-modality problem leads to inaccurate model prediction, especially for $\log p_\theta(\vx_{t+1})$.


\textbf{Salient Information-Based Guidance.}
Iterative sampling processes of diffusion models are often guided by external networks or themselves. Therein, salient information-based guidance has been actively explored~\cite{ho2022classifier,sag,improvedvq} for high-quality image synthesis.
Let $h$ be a salient information of $\vx$ and $\Bar{\vx}$ be a perturbed sample that lacks $h$. $h$ can be internal information within $\vx_t$ or an external condition, or both.
Given $h$, sampling $\vx$ to maximize $p(\Bar{\vx}|h)$.
However, for the correlation between the information and sample, $p(h|\Bar{\vx})$ also needs to be as large as possible~\cite{improvedvq}: $\log p(\Bar{\vx}|h) + s \log p(h|\Bar{\vx})$.
Using the Bayes' theorem, the equation can be represented as
\begin{equation}
    % \argmax_{\vx_t} [\log p_\theta(\vx_t) + (1+s)(\log p_\theta(\vx_t|h_t) - \log p_\theta(\vx_t))].
    \log p(\Bar{\vx}) + (1+s)(\log p(\Bar{\vx}|h) - \log p(\Bar{\vx})).
\end{equation}
Then the \cref{eq:sag} guides the sampling process toward enhancing the relevance of the sample and information $h$~\cite{sag}.
For example, in the setting $h=class$ and $\Bar{\vx}=\vx_t$, the \cref{eq:sag}
collapses to classifier-free guidance (CFG)~\cite{ho2022classifier,improvedvq}, which guides the sampling toward the given class distribution.


\begin{equation}
    \log p_\theta(\hat{\vx}_{0,t}) = \log p_\theta(\hat{\vx}_{0,t+1}|\vx_{t+2}) + (1+s)(\log p_\theta(\hat{\vx}_{0,t}|\vx_{t+1}) - \log p_\theta({\hat{\vx}}_{0,t+1}|\vx_{t+2}).
\end{equation}
Here, $h_t=\hat{\vx}_{0,t}-\hat{\vx}_{0,t+1}, \Bar{\vx}=\hat{\vx}_{0,t+1}$.

